Adaptive Approximate Policy Iteration

Model-free reinforcement learning algorithms combined with value function approximation have recently achieved impressive performance in a variety of application domains. However, the theoretical understanding of such algorithms is limited, and existing results are largely focused on episodic or discounted Markov decision processes (MDPs). In this work, we present adaptive approximate policy iteration (AAPI), a learning scheme which enjoys a $\tilde{O}(T^{2/3})$ regret bound for undiscounted, continuing learning in uniformly ergodic MDPs. This is an improvement over the best existing bound of $\tilde{O}(T^{3/4})$ for the average-reward case with function approximation. Our algorithm and analysis rely on online learning techniques, where value functions are treated as losses. The main technical novelty is the use of a data-dependent adaptive learning rate coupled with a so-called optimistic prediction of upcoming losses. In addition to theoretical guarantees, we demonstrate the advantages of our approach empirically on several environments.

==> Commands.tex <==
%\usepackage{pdfsync}

\usepackage{graphicx}

\newcommand{\todoy}[2][]{\todo[size=\scriptsize,color=red!20!white,#1]{Yasin: #2}}
\newcommand{\todoc}[2][]{\todo[size=\scriptsize,color=blue!20!white,#1]{Csaba: #2}}
\newcommand{\todonev}[2][]{\todo[size=\scriptsize,color=green!20!white,#1]{Nevena: #2}}
\newcommand{\todok}[2][]{\todo[size=\scriptsize,color=black!20!white,#1]{Kush: #2}}
\usepackage{amsmath,abbrevs}
\usepackage{amssymb}

% For citations
%\usepackage[round,sectionbib]{natbib}
% See:
% http://merkel.zoneo.net/Latex/natbib.php
%\bibpunct{[}{]}{;}{n}{}{,}

% THEOREMS -------------------------------------------------------
\newtheorem{theorem}{Theorem}[section]
\newtheorem{lemma}[theorem]{Lemma}
\newtheorem{proposition}[theorem]{Proposition}
\newtheorem{corollary}[theorem]{Corollary}
\newtheorem{definition}{Definition}[section]
\newtheorem{conjecture}[theorem]{Conjecture}
\newtheorem{remark}[theorem]{Remark}

%\newtheorem{remark}[thm]{Remark}

%\newcounter{assumption}%[section]
%\renewcommand{\theassumption}{A\arabic{assumption}}

%\newenvironment{ass}[1][]{\begin{trivlist}\item[] \refstepcounter{assumption}%
% {\bf Assumption\ \theassumption\ {\em (#1)} } }{%\par\nobreak\noindent\sl\ignorespaces}{%
% \ifvmode\smallskip\fi\end{trivlist}}
 
%\theoremstyle{definition}
\newtheorem{example}{Example}[section]

\usepackage{algorithm}
\usepackage{algorithmic}

\usepackage{color}
\usepackage{graphicx}
\usepackage{epstopdf}
%\usepackage{stmaryrd}
\usepackage{algorithm,algorithmic}
%\usepackage{verbatim}

%\usepackage{mathabx}

\usepackage{nicefrac}

%\usepackage{dsfont}
%\usepackage{subfig}
%\usepackage{small-headings}

% Turn on/off notes and descriptions of research problems
\newif\ifcomm
%\commfalse % also turns off internal todo comments
\commtrue

\newif\iflong
\longtrue
%\longfalse

% THEOREMS -------------------------------------------------------
%\newtheorem{theorem}{Theorem}[section]
%\newtheorem{lemma}[theorem]{Lemma}
%\newtheorem{proposition}[theorem]{Proposition}
%\newtheorem{corollary}[theorem]{Corollary}
%\newtheorem{definition}{Definition}[section]
%\newtheorem{conjecture}[theorem]{Conjecture}
%\newtheorem{remark}[theorem]{Remark}

%\newtheorem{remark}[thm]{Remark}

%\newcounter{assumption}%[section]
%\renewcommand{\theassumption}{A\arabic{assumption}}

%\newenvironment{assumption}[1][]{\begin{trivlist}\item[] \refstepcounter{assumption}%
% {\bf Assumption\ \theassumption\ {\em (#1)} } }{%\par\nobreak\noindent\sl\ignorespaces}{%
% \ifvmode\smallskip\fi\end{trivlist}}
 
%\theoremstyle{definition}
%\newtheorem{example}{Example}[section]

\newcommand{\vol}{\textsc{vol}} 

\newcommand{\vect}{\textsc{vec}} 
\newcommand{\mat}{\textsc{mat}} 

\newcommand{\cP}{{\cal P}} 
 
\newcommand{\norm}[1]{\left\Vert#1\right\Vert}
\newcommand{\abs}[1]{\left\vert#1\right\vert}
%\newcommand{\trace}{\mathop{\rm trace}}
\newcommand{\trace}{\mathop{\rm tr}}

\renewcommand{\natural}{\mathbb N}                   % Natural numbers
\newcommand{\N}{\mathbb N}                   % Natural numbers
\newcommand{\Real}{\mathbb R}                        % Real numbers
\newcommand{\R}{{\mathbb{R}}}                        % again..

%\newcommand{\Prob}[1]{{\mathbb P}\left(#1\right)}    % Probabilities; example: \Prob{X>\eps}<1-\delta
%\renewcommand{\P}{{\mathbb P}}                         % Probabilities when we want to control the parenthesis
\newcommand{\Prob}[1]{{\mathbf P}\left(#1\right)}    % Probabilities; example: \Prob{X>\eps}<1-\delta
\renewcommand{\P}{{\mathbf P}}                         % Probabilities when we want to control the parenthesis
\newcommand{\EE}[1]{{\mathbf E}\left[#1\right]}      % Expectations
\newcommand{\E}{{\mathbf E}}                         % Expectations  when we want to control the parenthesis
\newcommand{\Var}[1]{{\mathrm{Var}}\left[#1\right]}  % Variances
\newcommand{\Cov}{{\mathrm{Cov}}}  % Variances

\newcommand{\one}[1]{\mathbf 1 \left\{#1\right\}}           % Characteristic function

\newcommand{\eps}{\varepsilon}                       % Nice epsilon
\newcommand{\To}{\longrightarrow}
\newcommand{\ra}{\rightarrow}

\newcommand{\argmin}{\mathop{\rm argmin}}
\newcommand{\argmax}{\mathop{\rm argmax}}
\newcommand{\diag}{\mathop{\rm diag}}

\newcommand{\ip}[2]{\langle #1,#2 \rangle}
\newcommand{\eqdef}{\stackrel{\mbox{\rm\tiny def}}{=}}

\newcommand{\Tm}{T_\text{mix}}
% Shorthands I use for math environments
\newcommand{\beq}{\begin{equation}}
\newcommand{\eeq}{\end{equation}}

\newcommand{\RA}{$\Rightarrow$}
\ifcomm
   \newcommand\comm[1]{\textcolor{blue}{ #1}}
   \newcommand{\mtodo}[2]{\todo{{\bf #1}: #2}} % To add comments into the text; the first argument is "who", the second is "what"
   \def\here#1{{\bf $\langle\langle$#1$\rangle\rangle$}}

\else
   \newcommand\comm[1]{}
   \newcommand{\mtodo}[2]{}
   \def\here#1{}
\fi

\newcommand{\integer}{\mathbb{Z}}

%\renewcommand{\phi}{\varphi}


\newcommand{\cD}{{\cal D}}
\newcommand{\cE}{{\cal E}}
\newcommand{\cZ}{{\cal Z}}
\newcommand{\cX}{{\cal X}}
\newcommand{\cW}{{\cal W}}
\newcommand{\cC}{{\cal C}}
\newcommand{\cA}{{\cal A}}
\newcommand{\cY}{{\cal Y}}
\newcommand{\cB}{{\cal B}}
\newcommand{\cR}{{\cal R}}
\newcommand{\cT}{{\cal T}}
\newcommand{\cG}{{\cal G}}
\newcommand{\cF}{{\cal F}}
\newcommand{\cH}{{\cal H}}
\newcommand{\cM}{{\cal M}}
\newcommand{\cS}{{\cal S}}
\newcommand{\cV}{{\cal V}}
\newcommand{\cK}{{\cal K}}
\newcommand{\cN}{{\cal N}}

\newcommand{\mfrac}[2]{{}^{#1}/_{#2}}
\newcommand{\sfrac}{\nicefrac}

\newcommand{\e}{\mathbf{e}}
\newcommand{\bX}{\mathbf{X}}
\newcommand{\bI}{\mathbf{I}}
\newcommand{\bone}{\mathbf{1}}
\newcommand{\bzero}{\mathbf{0}}

\newcommand{\bB}{\mathbf{B}}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%\def\top{\intercal}

\def\eq#1{(\ref{eq-#1})}
\def\be{\begin{equation}}
\def\ee{\end{equation}}
\def\t{\theta}
\def\g{\gamma}
\def\a{\mathbf{a}}
\def\e{\mathbf{e}}
\def\y{\mathbf{y}}
\def\m{\boldsymbol{\mu}}
\def\A{\mathbf{A}}
\def\M{\mathbf{M}}
\def\1{\mathbf{1}}
%\def\P{\mathbf{P}}
\def\pa{\mathbf{p}_a}
\def\I{\mathbf{I}}
\def\p{{\boldsymbol{\pi}}}
\def\simplex{\Delta}
\def\A{\mathbf{A}}
\def\b{\mathbf{b}}
\def\c{\mathbf{c}}
\def\G{\mathbf{G}}
\def\O{\mathbf{O}}



\newname\controllermixture{{\rm \textsc{MDP-policy-mixture}}}
%\newname\controllermixtureperron{{\rm \textsc{Undiscounted-MDP-policy-mixture}}}
\newname\stableset{{\rm \textsc{independent-set}}}
 


